Towards Surveillance Video-and-Language Understanding: New Dataset, Baselines, and Challenges

Surveillance videos are an essential component of daily life with various critical applications, particularly in public security. However, current surveillance video tasks mainly focus on classifying and localizing anomalous events. Existing methods are limited to detecting and classifying the predefined events with unsatisfactory semantic understanding, although they have obtained considerable performance. To address this issue, we propose a new research direction of surveillance video-and-language understanding, and construct the first multimodal surveillance video dataset. We manually annotate the real-world surveillance dataset UCF-Crime with fine-grained event content and timing. Our newly annotated dataset, UCA (UCF-Crime Annotation), contains 23,542 sentences, with an average length of 20 words, and its annotated videos are as long as 110.7 hours. Furthermore, we benchmark SOTA models for four multimodal tasks on this newly created dataset, which serve as new baselines for surveillance video-and-language understanding. Through our experiments, we find that mainstream models used in previously publicly available datasets perform poorly on surveillance video, which demonstrates the new challenges in surveillance video-and-language understanding. To validate the effectiveness of our UCA, we conducted experiments on multimodal anomaly detection. The results demonstrate that our multimodal surveillance learning can improve the performance of conventional anomaly detection tasks. All the experiments highlight the necessity of constructing this dataset to advance surveillance AI. The link to our dataset is provided at: https://xuange923.github.io/Surveillance-Video-Understanding.

==> sec/5_futureworks.tex <==
-\section{Future works}

The experimental results from the aforementioned three multimodal tasks reveal that: there are still significant challenges in learning from multimodal surveillance video datasets. We will describe these challenges from two perspectives: the dataset and the model, and propose some future works.

\textbf{Dataset Challenges.}
Surveillance video datasets exhibit unique characteristics such as uneven image quality, complex backgrounds, and complex events when compared to previous multimodal video datasets. Because the collection of surveillance video data is still challenging, our UCA based on UCF-Crime, also suffers from insufficient data volumes. Consequently, the use of multimodal surveillance videos for research still faces significant challenges in terms of dataset quality and quantity. In the future, we can make more on the newly released surveillance videos~\cite{Cao_2023_CVPR}.

\textbf{Model Challenges.}
Current models have been well-trained on standard datasets, but their performance significantly deteriorates when applied to training on the UCA dataset. To mitigate these issues, it is crucial to retrain models on extensive amounts of data. Additionally, the model architecture must be modified and designed based on the unique characteristics of surveillance video datasets. In the future, we will pay more attention to research on capturing the dynamic characteristics of videos and locating events in long videos. 

